Online Learning with Imperfect Hints

We consider a variant of the classical online linear optimization problem in which at every step, the online player receives a "hint" vector before choosing the action for that round. Rather surprisingly, it was shown that if the hint vector is guaranteed to have a positive correlation with the cost vector, then the online player can achieve a regret of $O(\log T)$, thus significantly improving over the $O(\sqrt{T})$ regret in the general setting. However, the result and analysis require the correlation property at \emph{all} time steps, thus raising the natural question: can we design online learning algorithms that are resilient to bad hints? In this paper we develop algorithms and nearly matching lower bounds for online learning with imperfect directional hints. Our algorithms are oblivious to the quality of the hints, and the regret bounds interpolate between the always-correlated hints case and the no-hints case. Our results also generalize, simplify, and improve upon previous results on optimistic regret bounds, which can be viewed as an additive version of hints.

==> rel.tex <==
\section{Related work}
\subsection{Nika et al.~\cite{DBLP:conf/nips/DekelFHJ17}, following Hazan and Megiddo~\cite{DBLP:conf/colt/HazanM07}}

Consider the standard online linear optimization model, in which at every step, the algorithm plays a vector $x_t \in \cB_2(0,1)$ (unit $L_2$ ball in $d$ dimensions), and incurs a loss $\iprod{c_t, x_t}$, for some cost vector $c_t \in \mathbb{R}^d$.

Standard OLO admits an algorithm with regret $O(\sqrt{T})$, even on the unit ball. The hard instance is one in which the $c_t$ are random

Suppose that at every step, we know a ``hint" direction $v_t$ with the property that $\langle c_t, v_t \rangle \ge \alpha \cdot || c_t ||$, for some $\alpha >0$. Then there is an algorithm that achieves a regret of $O((\log T) / \alpha)$.

In the Hazan and Megiddo model, the hint vector is always some fixed coordinate direction, say $e_1$. 

The algorithm is quite simple: first select a vector in the orthogonal space by playing the Hedge algorithm with loss function $f(y_t ) = \langle d_t, y_t \rangle - \alpha \sqrt{1-\lVert y_t \rVert^2}$, where $d_t$ and $y_t$ are $[2:d]$ sub-vectors of $c_t, x_t$ respectively.

The analysis uses the fact that $f(\cdot)$ is exp-concave, with parameter $\alpha/d$.





